Spatially resolved Lyman-$\alpha$ emission around radio bright quasars

We use Southern African Large Telescope (SALT) to perform long-slit spectroscopic observations of 23 newly discovered radio-loud quasars (RLQs) at $2.7<z<3.3$. The sample consists of powerful AGN brighter than 200 mJy at 1.4 GHz and is selected on the basis of mid-infrared colors i.e., unbiased to the presence of dust. We report 7 confirmed and 5 tentative detections of diffuse Ly$\alpha$ emission in the sample. We present the properties of diffuse Ly$\alpha$ emission and discuss in detail its relationship to different quasar properties. We find strong dependence of Ly$\alpha$ halo detection rate on the extent of radio source, spectral luminosity of RLQ at 420 MHz ($L_{\rm 420MHz}$), presence of associated C IV absorption and nuclear He II emission line equivalent width. As seen in previous surveys, the FWHM of diffuse Ly$\alpha$ emission in the case of confirmed detections are much higher (i.e $>$1000 km/s in all, except one). Using the samples of high-$z$ radio-loud quasars and galaxies from literature, we confirm the correlation between the Ly$\alpha$ halo luminosity and its size with radio power ($L_{\rm 420MHz}$). The same quantities are found to be correlating weakly with the projected linear size of the radio emission. Our sample is the second largest sample of RLQs being studied for the presence of diffuse Ly$\alpha$ emission and fills in a redshift gap between previous such studies. Integral Field Spectroscopy is required to fully understand the relationship between the large scale radio emission and the overall distribution, kinematics and over density of Ly$\alpha$ emission in the field of these RLQs.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
